Predictive calibration for digital sun sensors using sparse submanifold convolutional neural networks

Recent developments in AI techniques for space applications mirror the success achieved in terrestrial applications. Machine learning, which excels in data rich environments, is particularly well suited to space-based computer vision applications, such as space optical attitude sensing. Of these sensors, digital sun sensors (DSS) are one of the most common and important sensors for spacecraft attitude determination. The main challenge in using the DSS for attitude estimation are sensor errors, which limit the overall achievable estimation accuracy. However, the traditional sun sensor calibration process is costly, slow, labor-intensive and inefficient. These limitations motivate the use of AI techniques to enable more accurate and efficient DSS calibration. The objective of this work is to develop an end-to-end predictive calibration methodology for digital sun sensors to solve 2-axis state estimates utilizing a sparse submanifold convolutional neural network (SSCNN). We find that the proposed framework can achieve state-of-the-art performance on synthetic data with a mean accuracy of 0.005{\deg} for the two sun angle estimates. Furthermore, the model is highly capable of implicitly learning complex noise patterns and handling mixed noise types, thereby greatly improving the model robustness and accuracy to real-world applications. The main contributions of this work are: (1) the first application (to our knowledge) of a CNN regression model to the problem of DSS predictive calibration, (2) the introduction of a fused end-to-end training approach for DSS calibration, (3) the creation of a publicly available physics-informed synthetic dataset and simulation for DSS training images, and (4) the evaluation of the performance of the deep learning approach for various mask configurations.

==> layers/init.tex <==
%\ProvidesPackage{init}
\usetikzlibrary{quotes,arrows.meta}
\usetikzlibrary{positioning}

\def\edgecolor{rgb:blue,4;red,1;green,4;black,3}
\newcommand{\midarrow}{\tikz \draw[-Stealth,line width =0.8mm,draw=\edgecolor] (-0.3,0) -- ++(0.3,0);}

\usepackage{Ball}
\usepackage{Box}
\usepackage{RightBandedBox}
